Towards Offloadable and Migratable Microservices on Disaggregated Architectures: Vision, Challenges, and Research Roadmap

Microservice and serverless computing systems open up massive versatility and opportunity to distributed and datacenter-scale computing. In the meantime, the deployments of modern datacenter resources are moving to disaggregated architectures. With the flourishing growths from both sides, we believe this is high time to write this vision paper to propose a potential research agenda to achieve efficient deployments, management, and executions of next-generation microservices on top of the emerging disaggregated datacenter architectures. In particular, we envision a critical systems research direction of designing and developing offloadable and migratable microservices on disaggregated architectures. With this vision, we have surveyed the recent related work to demonstrate the importance and necessity of researching it. We also outline the fundamental challenges that distributed systems and datacenter-scale computing research may encounter. We further propose a research roadmap to achieve our envisioned objectives in a promising way. Within the roadmap, we identify potential techniques and methods that can be leveraged.

==> Makefile <==
TARGETS: all

# Make file for latex building
.PHONY: all clean

all: pdf

pdf: 
	for i in 1 2 3; do \
		bibtex header; \
		pdflatex header; \
		done

clean:
	rm -f header.bak header.aux header.blg header.log header.dvi header.ps header.pdf *~ Text/*.bak header.out

